Diffusion Parameter Estimation for the Homogenized Equation

We construct a novel estimator for the diffusion coefficient of the limiting homogenized equation, when observing the slow dynamics of a multiscale model, in the case when the slow dynamics are of bounded variation. Previous research suggests subsampling the data on fixed intervals and computing the corresponding quadratic variation. However, to achieve optimality, this approach requires knowledge of scale separation variable $\epsilon$. Instead, we suggest computing the quadratic variation corresponding to the local extrema of the slow process. Our approach results to a natural subsampling and avoids the issue of choosing a subsampling rate. We prove that the estimator is asymptotically unbiased and we numerically demonstrate that its $L_2$-error is of order ${\mathcal O}(\epsilon^2)$.

==> Estimator.tex <==


\section{The Estimator}
\label{sec: Types}

If we observed the homogenized equation $X$ rather than the slow process $x^\epsilon$, then it is well known that $\Sigma$ can be estimated efficiently from the quadratic variation 
\begin{equation}
D_{2}\left(X\right)_{T}=\lim_{\text{mesh}(\pi_{n}([0.T]))\rightarrow0}\left(\sum_{t_{i}\in\pi_{(n)}([0,T])}(\Delta X((t_{i}))^{2}\right)^{1/2} = \Sigma \cdot\sqrt{T},
\end{equation}
where $\Delta X(t_{i}):=X(t_{i})-X(t_{i-1})$ and $\pi_{(n)}([0,T])=\left\{ 0=t_{0},t_{1},...,t_{n}=T\right\} $ a partition of size $n+1$ on the fixed time interval $[0,T]$ with $\text{mesh}(\pi_{n}([0,T])):=\max_{1\leq i\leq n}(t_{i}-t_{i-1})$. However, if instead we use the bounded variation process $x^\epsilon$, its quadratic variation is be $0$, i.e. $D_{2}\left(x^\epsilon\right)_{T} = 0$. Thus, because of the mismatch between model and data, the standard estimator is not longer useful. 

To avoid this problem, in \cite{papavasiliou2011coarse}, the autor suggests using the total $2$-variation of the process (see \cite{lyons2002system}) rather than the quadratic variation, defined as 
\begin{equation}
D_{2}^{\text{Total}}\left(x^\epsilon\right)_{T}=\sup_{\mathcal{D}([0,T])}\left(\sum_{t_{i}\in\mathcal{D}([0,T])}(x^\epsilon_{t_{i}}-x^\epsilon_{t_{i-1}})^{2}
\right)^{1/2},
\end{equation}
By taking the supremum over all partitions, the total $2$-variation can only be zero if the path $x^\epsilon$ is constant, so it maintains much more information than quadratic variation. In the case of a piecewise linear path, the supremum is achieved at a subset of the extemal points of the path \cite{Driver13}. However, this is still computationally very inefficient and causes a lot of technical difficulties, which is what limited \cite{papavasiliou2011coarse} to the analysis to the mutliscale Ornstein-Uhlenbeck model.

In this paper, we consider a simplification of the total $2$-variation that we will call the Extrema Quadratic Variation, defined as follows:
\begin{defn}
\label{subsec: ExtQV}
Let $x(t):[0,T]\rightarrow\mathbb{R}$ be a real\textendash valued
continuous path and let $x_{n}(t)$ be the piecewise linear approximation
of $x$ on a homogeneous grid of size $n+1$. We define the {\it Extrema Quadratic Variation} (ExtQV) of the path $x$
on the time interval $[0,T]$ as
\begin{equation}
D_{2}^{\text{Ext}}\left(x\right)_{T}=\lim_{n\rightarrow\infty}\left(D_{2}^{\text{Ext}}\left(x_{n}\right)_{T}\right)=\lim_{n\rightarrow\infty}\left(\sum_{\tau_{i}\in\mathcal{E}_{(n)}([0,T])}(\Delta x_{n}(\tau_{i}))^{2}\right)^{1/2},
\end{equation}
where $\mathcal{E}_{(n)}([0,T])=\left\{0= \tau_{0},\tau_{1},...,\tau_{k}=T\right\} $
is the set of local extremals of $x_{n}(t)$ and $\Delta x_{n}(\tau_{i}):=x_{n}(\tau_{i})-x_{n}(\tau_{i-1})$,
$i=1,...,k$.
\end{defn}


In other words, let $\pi_{n}([0,T]):=\{t_{0},t_{1},...,t_{n}\}=\left\{ i\frac{T}{n},i=0,...,n\right\} $
an equally subdivided partition of $[0,T]$, with time step $\delta:=T/n$
. We say that a point $t_{i}$ in $\pi_{n}([0,T])$ is an extremal
point and we write $t_{i}\in\mathcal{E}_{(n)}([0,T])$ if $\Delta x_{n}(t_{i})\Delta x_{n}(t_{i+1})=\left(x_{t_{i}}-x_{t_{i-1}}\right)\left(x_{t_{i+1}}-x_{t_{i}}\right)<0$.

Figure \ref{fig: extremal_point} illustrates an example of an extremal point. The point $t_{i}$ is an extremal point since $\Delta x_{n}(t_{i})<0$ and  $\Delta x_{n}(t_{i+1})>0$.

\begin{figure}[t]
\begin{center}
\begin{tikzpicture}
\draw[->] (0,0) -- (6,0) node[anchor=north] {$t$};
\draw	(1,0) node[anchor=north] {$t_{i-1}$}
		(3,0) node[anchor=north] {$t_{i}$}
		(5,0) node[anchor=north] {$t_{i+1}$};
\draw[->] (0,0) -- (0,4) node[anchor=east] {$x$};
\draw[thick] (1,1) -- (3,3) -- (5,2);
\draw[dotted] (1,0) -- (1,1);
\draw[dotted] (3,0) -- (3,3);
\draw[dotted] (5,0) -- (5,2);
\draw	(0,1) node[anchor=east] {$x_{t_{i-1}}$}
		(0,3) node[anchor=east] {$x_{t_{i}}$}
		(0,2) node[anchor=east] {$x_{t_{i+1}}$};
\draw[dotted] (0,1) -- (5,1);
\draw[dotted] (0,2) -- (5,2);
\draw[dotted] (0,3) -- (5,3);
\draw[dotted] (5,2) -- (5,3);
\draw[dotted] (3,1) -- (3,3);
\draw	(5,2.5) node[anchor=west] {$\Delta x_{t_{i+1}}$}
		(3,2) node[anchor=west] {$\Delta x_{t_{i}}$};
\end{tikzpicture}
\end{center}
\caption[Graphical representation of an extremal point.]{Graphical representation of an extremal point.}\label{fig: extremal_point}
\end{figure}

The extremal partition corresponding to $x_n$  will be denoted as  $\mathcal{E}_{(x_n)}{([0,T])}$ and is defined as the set of local extremals points from the initial partition $\pi_{(n)}([0,T])$. We will use the letter $t$ to denote points in the origianl partition $\pi_{(n)}([0,T])\}$ and the letter $\tau$ to denote points in the extremal partition  $mathcal{E}_{(x_n)}{([0,T])}\}$. The computation of the quadratic variation requires
the consideration of all the increments of the original path whereas the extrema quadratic variation the increments of the extremal path. In Figure \ref{fig: OriginalVsExtrema} we illustrate graphically an example of an extremal path. The black line is the original path and the red line is the corresponding extremal path.

\begin{figure}[H]
\begin{center}
\includegraphics[width=11cm,height=6.6cm]{extrema_var.pdf}
\end{center}
\caption[Graphical representation of an extremal path.]{Graphical representation of an extremal path: the original path (black line) and the extremal path (red line).}
\label{fig: OriginalVsExtrema}
\end{figure}

An alternative way to compute the (ExtQV) is presented
below. This way appears
to be very useful in the analytic computation of the expectation of the
(ExtQV). Formula \eqref{eq: ext_QV} suggests that the (ExtQV) is the sum of
squared returns of the original process plus two times the product
of those increments such that the consecutive products of the increments
between these two are all positive.

In what follows we define $C_n(i,j)$ as the subspace of the space of piecewise linear paths on $\pi_n([0,T])$ (denoted by $PL(\pi_n([0,T]))$ that are monotonic between $t_{i-1}$ and $t_j$ with $i<j$, i.e.
$$
C_n(i,j):=\{ z_n \in PL(\pi_n([0,T])): \Delta z_{n}(t_{i})\Delta z_{n}(t_{i+1})>0,...,\Delta z_{n}(t_{i})\Delta z_{n}(t_{j})>0\}.
$$
Using this notation, the (ExtQV) of a piecewise linear process $x_n$ is expressed as follows:
\begin{align}
D_{2}^{\text{Ext}}(x_{n})_{T}& =D_{2}(x_{n})_{T}+2\sum_{i=1}^{j-1}\sum_{j=2}^{n}\bigg(\Delta x_{n}(t_{i})\Delta x_{n}(t_{j})\mathbf{1}_{C_n(i,j)}\left(x_n\right)\bigg), \label{eq: ext_QV}
\end{align}
where
  \[
    \mathbf{1}_{C_n(i,j)}\left(x_n\right) = \left\{\begin{array}{lr}
        1, & \text{if } x_n\in C_n(i,j),\\
        0, & \text{otherwise.}
        \end{array}\right.
  \]




